Near optimal finite time identification of arbitrary linear dynamical systems

We derive finite time error bounds for estimating general linear time-invariant (LTI) systems from a single observed trajectory using the method of least squares. We provide the first analysis of the general case when eigenvalues of the LTI system are arbitrarily distributed in three regimes: stable, marginally stable, and explosive. Our analysis yields sharp upper bounds for each of these cases separately. We observe that although the underlying process behaves quite differently in each of these three regimes, the systematic analysis of a self--normalized martingale difference term helps bound identification error up to logarithmic factors of the lower bound. On the other hand, we demonstrate that the least squares solution may be statistically inconsistent under certain conditions even when the signal-to-noise ratio is high.

==> content/a.tex <==
\newpage
\onecolumn
\section{Appendix}
\label{appendix_matrix}
\begin{prop}
	\label{psd_result_2}
	Let $P, V$ be a psd and pd matrix respectively and define $\bar{P} = P + V$. Let there exist some matrix $Q$ for which we have the following relation
	\[
	||\bar{P}^{-1/2} Q|| \leq \gamma
	\]
	For any vector $v$ such that $v^{\prime} P v = \alpha, v^{\prime} V v =\beta$ it is true that
	\[
	||v^{\prime}Q|| \leq \sqrt{\beta+\alpha} \gamma 
	\]
\end{prop}
\begin{proof}
	Since 
	\[
	||\bar{P}^{-1/2} Q||_2^2 \leq \gamma^2 	
	\] 
	for any vector $v \in \Sc^{d-1}$ we will have 
	\[
	\frac{v^{\prime} \bar{P}^{1/2}\bar{P}^{-1/2} Q Q^{\prime}\bar{P}^{-1/2}\bar{P}^{1/2} v}{v^{\prime} \bar{P} v} \leq \gamma^2
	\]
	and substituting $v^{\prime} \bar{P} v = \alpha + \beta$ gives us
	\begin{align*}
	{v^{\prime}  Q Q^{\prime} v} &\leq \gamma^2{v^{\prime} \bar{P} v} \\
	&= (\alpha + \beta) \gamma^2
	\end{align*}
\end{proof}

%\begin{prop}
%	\label{gramian_lb}
%	Let $1 - C/T \leq \rho_i(A) \leq 1 + C/T$. Then there exists $\alpha(A)$ depending only on $A$ such that
%	\[
%		\sigma_{\min}(\Gamma_T(A)) \geq T \alpha(A)
%	\]	
%\end{prop}
%\begin{proof}
%	First we note a property of stable matrices, \textit{i.e.}, whenever $C$ is stable $\Gamma_{\infty}(C)$ exists and is finite. Then for any $k$
%	\[
%	C^k C^{k \prime} \preceq \Gamma_{\infty}(C) - I
%	\]
%	As a result $||C^k|| \leq \sqrt{\sigma_{\max}(\Gamma_{\infty}(C)) - 1}$. For two psd matrices $A, B$ we have from Weyl's inequality
%	\[
%	\sigma_{\min}(D + B) \geq \sigma_{\min}(D) + \sigma_{\min}(B)
%	\]
%	Now we know that 
%	\[
%	\Gamma_{T}(A) = \sum_{k=0}^T A^k A^{k \prime}
%	\]
%	and it follows that 
%	\[
%	\sigma_{\min}(\Gamma_T(A)) \geq \sum_{k=0}^T \sigma_{\min}(A^k A^{k \prime})
%	\]
%	To lower bound $\sigma_{\min}(A)$ we upper bound $\sigma_{\max}(A^{-1})$. Since $\rho_{\min} \geq 1 -\frac{C}{T} > 1/2$ we have $\frac{A}{1 - 2C/T}$ has all eigenvalues that are greater than $1$ in absolute value. This implies that $\tilde{A}^{-1} = (1 - 2C/T) A^{-1}$ is stable. As a result we have 
%	\[
%	||\tilde{A}^{-k}|| \leq \sqrt{\sigma_{\max}(\Gamma_{\infty}(\tilde{A})) - 1}
%	\]
%	
%	Then for every $k \leq T$
%	\begin{align*}
%	\sigma_{\max}(\tilde{A}^{-k}) &= (1-2C/T)^k \sigma_{\max}(A^{-1}) \\
%	&\overset{(a)}{\leq} C(\tilde{A}^{-1}) \rho_{\max}(\tilde{A}^{-k}) \\
%	&\leq C(\tilde{A}^{-1}) \frac{1}{\rho_{\min}(A^{k})} \\
%	\sigma_{\min}(A^{k})&\overset{(b)}{\geq} \frac{e^{-C}}{C(A)} 
%	\end{align*}
%	$(a)$ follows from [Cite Recht Paper]. $(b)$ is true for every $k \leq T$ because $\rho_{\min} \geq 1-C/T \implies \rho_{\min}^T \geq e^{-C}$. Now we get that 
%	\[
%	\sigma_{\min}(\Gamma_T(A)) \geq \frac{e^{-C}T}{C(A)}
%	\]
%\end{proof}	
\begin{prop}
	\label{inv_jordan}
Consider a Jordan block matrix $J_d(\lambda)$ given by \eqref{jordan}, then $J_d(\lambda)^{-k}$ is a matrix where each off--diagonal (and the diagonal) has the same entries, \textit{i.e.},
	\begin{equation}
	J_d(\lambda)^{-k} =\begin{bmatrix}
	a_1 & a_2 &  a_3 & \hdots & a_d \\
	0 & a_1 & a_2 & \hdots & a_{d-1} \\
	\vdots & \vdots & \ddots & \ddots & \vdots \\
	0 & \hdots & 0 & a_1 & a_2 \\
	0 & 0 & \hdots & 0 & a_1  
	\end{bmatrix}_{d \times d}
	\end{equation}
for some $\{a_i\}_{i=1}^d$.
\end{prop}
\begin{proof}
	$J_d(\lambda) = (\lambda I + N)$ where $N$ is the matrix with all ones on the $1^{st}$ (upper) off-diagonal. $N^k$ is just all ones on the $k^{th}$ (upper) off-diagonal and $N$ is a nilpotent matrix with $N^d = 0$. Then
	\begin{align*}
	(\lambda I + N)^{-1} &= (\sum_{l=0}^{d-1} (-1)^{l}\lambda^{-l-1}N^{l}) \\
	(-1)^{k-1}(k-1 )!(\lambda I + N)^{-k} &= \Big(\sum_{l=0}^{d-1} (-1)^{l}\frac{d^{k-1}\lambda^{-l-1}}{d \lambda^{k-1}}N^{l}\Big) \\
	&= \Big(\sum_{l=0}^{d-1} (-1)^{l}c_{l, k}N^{l}\Big) 
	\end{align*} 

and the proof follows in a straightforward fashion.
\end{proof}
\begin{prop}
	\label{reg_invertible}
Let $A$ be a regular matrix and $A = P^{-1} \Lambda P$ be its Jordan decomposition. Then
\[
\inf_{||a||_2 = 1}||\sum_{i=1}^d a_i \Lambda^{-i+1}||_2 > 0
\]
Further $\phi_{\min}(A) > 0$ where $\phi_{\min}(\cdot)$ is defined in Definition~\ref{outbox}.
\end{prop}
\begin{proof}
	When $A$ is regular, the geometric multiplicity of each eigenvalue is $1$. This implies that $A^{-1}$ is also regular. Regularity of a matrix $A$ is equivalent to the case when minimal polynomial of $A$ equals characteristic polynomial of $A$ (See Section~\ref{lemmab} in appendix), \textit{i.e.},
	\begin{align*}
	\inf_{||a||_2 = 1}||\sum_{i=1}^d a_i A^{-i+1}||_2  &> 0
	\end{align*}
	Since $A^{-j} = P^{-1} \Lambda^{-j} P$ we have
	\begin{align*}
	\inf_{||a||_2 = 1}||\sum_{i=1}^d a_i P^{-1}\Lambda^{-i+1}P||_2 &> 0 \\
	\inf_{||a||_2 = 1}||\sum_{i=1}^d a_i P^{-1}\Lambda^{-i+1}||_2 \sigma_{\min}(P) &> 0 \\
	\inf_{||a||_2 = 1}||\sum_{i=1}^d a_i \Lambda^{-i+1}||_2 \sigma_{\min}(P) \sigma_{\min}(P^{-1}) &> 0 \\
	\inf_{||a||_2 = 1}||\sum_{i=1}^d a_i \Lambda^{-i+1}||_2 &>0	
	\end{align*}
	Since $\Lambda$ is Jordan matrix of the Jordan decomposition, it is of the following form
	\begin{equation}
	\Lambda  =\begin{bmatrix}
	J_{k_1}(\lambda_1) & 0 & \hdots & 0 &0 \\
	0 & J_{k_2}(\lambda_2) & 0 & \hdots &0  \\
	\vdots & \vdots & \ddots & \ddots & \vdots \\
	0 & \hdots & 0 & J_{k_{l}}(\lambda_l) & 0 \\
	0 & 0 & \hdots & 0 & J_{k_{l+1}}(\lambda_{l+1})
	\end{bmatrix}
	\end{equation} 
	where $J_{k_i}(\lambda_i)$ is a $k_i \times k_i$ Jordan block corresponding to eigenvalue $\lambda_i$. Then
	\begin{equation}
	\Lambda^{-k}  =\begin{bmatrix}
	J^{-k}_{k_1}(\lambda_1) & 0 & \hdots & 0 &0 \\
	0 & J^{-k}_{k_2}(\lambda_2) & 0 & \hdots &0  \\
	\vdots & \vdots & \ddots & \ddots & \vdots \\
	0 & \hdots & 0 & J^{-k}_{k_{l}}(\lambda_l) & 0 \\
	0 & 0 & \hdots & 0 & J^{-k}_{k_{l+1}}(\lambda_{l+1})
	\end{bmatrix}
	\end{equation} 	
Since $||\sum_{i=1}^d a_i \Lambda^{-i+1}||_2 >0$, without loss of generality assume that there is a non--zero element in $k_1 \times k_1$ block. This implies 
\begin{align*}
||\underbrace{\sum_{i=1}^d a_i J_{k_1}^{-i+1}(\lambda_1)}_{=S}||_2  > 0
\end{align*}
By Proposition~\ref{inv_jordan} we know that each off--diagonal (including diagonal) of $S$ will have same element. Let $j_0 = \inf{\{j | S_{ij} \neq 0\}}$ and in column $j_0$ pick the element that is non--zero and highest row number, $i_0$. By design $S_{i_0, j_0} > 0$ and further
$$S_{k_1 -(j_0 - i_0), k_1} = S_{i_0, j_0}$$ 
because they are part of the same off--diagonal (or diagonal) of $S$. Thus the row $k_1 - (j_0 - i_0)$ has only one non--zero element because of the minimality of $j_0$.

We proved that for any $||a||=1$ there exists a row with only one non--zero element in the matrix $\sum_{i=1}^d a_i \Lambda^{-i+1}$. This implies that if $v$ is a vector with all non--zero elements, then $||\sum_{i=1}^d a_i \Lambda^{-i+1} v||_2 > 0$, \textit{i.e.},
\begin{align*}
\inf_{||a||_2 = 1}||\sum_{i=1}^d a_i \Lambda^{-i+1} v ||_2 &> 0 
\end{align*}
This implies
\begin{align*}
\inf_{||a||_2 = 1}||[v, \Lambda^{-1} v, \ldots, \Lambda^{-d+1}v] a||_2 &> 0\\
\sigma_{\min}([v, \Lambda^{-1} v, \ldots, \Lambda^{-d+1}v]) &> 0 \\
\end{align*}
By Definition~\ref{outbox} we have
\begin{align*}
\phi_{\min}(A) &> 0
\end{align*}
\end{proof}
\begin{prop}[Corollary 2.2 in~\cite{ipsen2011determinant}]
	\label{det_lb}
	For any positive definite matrix  $M$ with diagonal entries $m_{jj}$, $1 \leq j \leq d$ and $\rho$ is the spectral radius of the matrix $C$ with elements
	\begin{align*}
	c_{ij} &= 0 \hspace{3mm} \text{if } i=j \\
	 &=\frac{m_{ij}}{\sqrt{m_{ii}m_{jj}}}  \hspace{3mm} \text{if } i\neq j
	\end{align*}
	then 
	\begin{align*}
	0 < \frac{\prod_{j=1}^d m_{jj} - \text{det}(M)}{\prod_{j=1}^d m_{jj}} \leq 1 - e^{-\frac{d \rho^2}{1+\lambda_{\min}}}
	\end{align*}
	where $\lambda_{\min} = \min_{1 \leq j \leq d} \lambda_j(C)$.
\end{prop}
\begin{prop}
	\label{gramian_lb}
	Let $1 - C/T \leq \rho_i(A) \leq 1 + C/T$ and $A$ be a $d \times d$ matrix. Then there exists $\alpha(d)$ depending only on $d$ such that for every $8 d \leq t \leq T$
	\[
	\sigma_{\min}(\Gamma_t(A)) \geq t \alpha(d) 
	\]	
\end{prop}
\begin{proof}
	Since $A = P^{-1} \Lambda P$ where $\Lambda$ is the Jordan matrix. Since $\Lambda$ can be complex we will assume that adjoint instead of transpose. This gives
	\begin{align*}
	\Gamma_T(A) &= I + \sum_{t=1}^T A^t (A^{t})^{\prime} \\
		&= I + P^{-1}\sum_{t=1}^T \Lambda^tPP^{\prime} (\Lambda^t)^{*} P^{-1 \prime} \\
		&\succeq I + \sigma_{\min}(P)^2P^{-1}\sum_{t=1}^T \Lambda^t(\Lambda^t)^{*} P^{-1 \prime} 
	\end{align*}
Then this implies that 
\begin{align*}
\sigma_{\min}(	\Gamma_T(A)) &\geq 1 +\sigma_{\min}(P)^2 \sigma_{\min}(P^{-1}\sum_{t=1}^T \Lambda^t(\Lambda^t)^{\prime} P^{-1 \prime}) \\
&\geq 1 + \sigma_{\min}(P)^2 \sigma_{\min}(P^{-1})^2\sigma_{\min}(\sum_{t=1}^T \Lambda^t(\Lambda^t)^{\prime} ) \\
&\geq 1 + \frac{\sigma_{\min}(P)^2}{\sigma_{\max}(P)^2}\sigma_{\min}(\sum_{t=1}^T \Lambda^t(\Lambda^t)^{\prime} )
\end{align*}

Now 
\begin{align*}
\sum_{t=0}^T \Lambda^t(\Lambda^t)^{*} &= \begin{bmatrix}
\sum_{t=0}^T J^{t}_{k_1}(\lambda_1)(J^{t}_{k_1}(\lambda_1))^{*} & 0 & \hdots & 0  \\
0 & \sum_{t=1}^T J^{t}_{k_2}(\lambda_2)(J^{t}_{k_2}(\lambda_2))^{*} & 0 & \hdots   \\
\vdots & \vdots & \ddots & \ddots \\
0 & \hdots & 0 & \sum_{t=1}^T J^{t}_{k_{l}}(\lambda_l) (J^{t}_{k_l}(\lambda_l))^{*} 
\end{bmatrix}
\end{align*}

Since $\Lambda$	is block diagonal we only need to worry about the least singular value corresponding to some block. Let this block be the one corresponding to $J_{k_1}(\lambda_1)$, \textit{i.e.},
\begin{equation}
\sigma_{\min}(\sum_{t=0}^T \Lambda^t(\Lambda^t)^{*} ) =\sigma_{\min}(\sum_{t=0}^T J^{t}_{k_1}(\lambda_1)(J^{t}_{k_1}(\lambda_1))^{*}) \label{bnd_1}
\end{equation}
% Now, $\lambda_1$ might be complex but using a result in~\cite{erxiong1994691} we see that we can focus on $|\lambda_1|$. This is because there exists a complex unitary diagonal similarity transform, $D$, that ensures 
%\[
%D^{*}\sum_{t=1}^T J^{t}_{k_1}(\lambda_1)(J^{t}_{k_1}(\lambda_1))^{*}D = \sum_{t=1}^T J^{t}_{k_1}(|\lambda_1|)(J^{t}_{k_1}(|\lambda_1|))^{\prime}
%\]

Define $B =  \sum_{t=0}^T J^{t}_{k_1}(\lambda_1)(J^{t}_{k_1}(\lambda_1))^{*}$. Note that $J_{k_1}(\lambda_1) = (\lambda_1 I + N)$ where $N$ is the nilpotent matrix that is all ones on the first off--diagonal and $N^{k_1} = 0$. Then 
\begin{align*}
(\lambda_1 I + N)^t &= \sum_{j=0}^t {t \choose j} \lambda_1^{t-j}N^{j} \\
(\lambda_1 I + N)^t((\lambda_1 I + N)^t)^{*} &= \Big(\sum_{j=0}^t {t \choose j} \lambda_1^{t-j}N^{j}\Big)\Big(\sum_{j=0}^t {t \choose j} (\lambda_1^{*})^{t-j}N^{j \prime}\Big) \\
&= \sum_{j=0}^t {t \choose j}^2 |\lambda_1|^{2(t-j)} \underbrace{N^j (N^j)^{\prime}}_{\text{Diagonal terms}} + \sum_{j \neq k}^{j=t, k=t} {t \choose k}{t \choose j} \lambda_1^j (\lambda_1^{*})^{k} N^j (N^k)^{\prime} \\
&= \sum_{j=0}^t {t \choose j}^2 |\lambda_1|^{2(t-j)} \underbrace{N^j (N^j)^{\prime}}_{\text{Diagonal terms}} + \sum_{j > k}^{j=t, k=t} {t \choose k}{t \choose j} \lambda_1^j (\lambda_1^{*})^{k} N^j (N^k)^{\prime} \\
&+ \sum_{j< k}^{j=t, k=t} {t \choose k}{t \choose j} \lambda_1^j (\lambda_1^{*})^{k} N^j (N^k)^{\prime} \\
&= \sum_{j=0}^t {t \choose j}^2 |\lambda_1|^{2(t-j)} \underbrace{N^j (N^j)^{\prime}}_{\text{Diagonal terms}} + \sum_{j > k}^{j=t, k=t} {t \choose k}{t \choose j} \underbrace{|\lambda_1|^{2k} \lambda_1^{j-k} N^{j-k} N^k(N^k)^{\prime}}_{\text{On $(j-k)$ upper off--diagonal}} \\
&+ \sum_{j< k}^{j=t, k=t} {t \choose k}{t \choose j} \underbrace{|\lambda_1|^{2j} (\lambda_1^{*})^{k-j} N^j(N^{j})^{\prime} (N^{j-k})^{\prime}}_{\text{On $(k-j)$ lower off--diagonal}}
\end{align*}
Let $\lambda_1 = r e^{i\theta}$, then similar to~\cite{erxiong1994691}, there is $D = \text{Diag}(1, e^{-i\theta}, e^{-2i\theta}, \ldots, e^{-i(k_1-1)\theta})$ such that 
\[
\underbrace{D (\lambda_1 I + N)^t((\lambda_1 I + N)^t)^{*} D^{*}}_{\text{Real Matrix}}
\]
Observe that any term on $(j-k)$ upper off--diagonal of $(\lambda_1 I + N)^t((\lambda_1 I + N)^t)^{*}$ is of the form $r_0 e^{i(j-k)\theta}$. In the product $D (\lambda_1 I + N)^t((\lambda_1 I + N)^t)^{*} D^{*}$ any term on the $(j-k)$ upper off diagonal term now looks like $e^{-ij\theta + ik\theta} r_0 e^{i(j-k)\theta} = r_0$, which is real. Then we have 
\begin{align}
D (\lambda_1 I + N)^t((\lambda_1 I + N)^t)^{*} D^{*} &= \sum_{j=0}^t {t \choose j}^2 |\lambda_1|^{2(t-j)} \underbrace{N^j (N^j)^{\prime}}_{\text{Diagonal terms}} + \sum_{j > k}^{j=t, k=t} {t \choose k}{t \choose j} \underbrace{|\lambda_1|^{2k} |\lambda_1|^{j-k} N^{j-k} N^k(N^k)^{\prime}}_{\text{On $(j-k)$ upper off--diagonal}} \nonumber\\
&+ \sum_{j< k}^{j=t, k=t} {t \choose k}{t \choose j} \underbrace{|\lambda_1|^{2j} |\lambda_1|^{k-j} N^j(N^{j})^{\prime} (N^{k-j})^{\prime}}_{\text{On $(k-j)$ lower off--diagonal}} \label{real}
\end{align}
Since $D$ is unitary and $D (\lambda_1 I + N)^t((\lambda_1 I + N)^t)^{*} D^{*} =(|\lambda_1| I + N)^t((|\lambda_1| I + N)^t)^{\prime} $, we can simply work with the case when $\lambda_1 > 0$ and real, as the singular values remain invariant under unitary transformations. Now we show the growth of $ij^{th}$ term of the product $D (\lambda_1 I + N)^t((\lambda_1 I + N)^t)^{*} D^{*})$,
Define $B=\sum_{t=1}^T (|\lambda_1| I + N)^t((|\lambda_1| I + N)^t)^{\prime}$
\begin{align}
B_{ll} &=\sum_{t=1}^T [(\lambda_1 I + N)^t((\lambda_1 I + N)^t)^{*}]_{ll} \\
&= \sum_{t=1}^T \sum_{j=0}^{k_1-l} {t \choose j}^2 |\lambda_1|^{2(t-j)} \label{bll}
\end{align}
Since $1-C/T \leq |\lambda_1| \leq 1+C/T$, then for every $t \leq T$ we have 
$$e^{-C} \leq |\lambda_1|^t \leq e^{C}$$
Then 
\begin{align}
B_{ll} &= \sum_{t=1}^T \sum_{j=0}^{k_1-l} {t \choose j}^2 |\lambda_1|^{2(t-j)} \nonumber\\
&\geq e^{-2C} \sum_{t=1}^T \sum_{j=0}^{k_1-l} {t \choose j}^2 \nonumber\\
& \geq e^{-2C} \sum_{t=T/2}^T \sum_{j=0}^{k_1-l} {t \choose j}^2 \geq e^{-C} \sum_{t=T/2}^T c_{k_1} \frac{t^{2k_1-2l+2} - 1}{t^2 - 1}  \geq C(k_1) T^{2k_1 - 2l+1} \label{lb}
\end{align}
An upper bound can be achieved in an equivalent fashion. 
\begin{align}
B_{ll} &= \sum_{t=1}^T \sum_{j=0}^{k_1-l} {t \choose j}^2 |\lambda_1|^{2(t-j)} \nonumber\\
& \leq e^{2C} T \sum_{j=0}^{k_1-l} T^{2j} \leq C(k_1) T^{2k_1 - 2l + 1} \label{ub1}
\end{align}
Similarly, for any $B_{k,k+l} $ we have
\begin{align}
B_{k, k+l} &=\sum_{t=1}^T \sum_{j=0}^{k_1-k - l} {t \choose j}{t \choose j+l} |\lambda_1|^{2j} |\lambda_1|^{l}  \\
&\geq \sum_{t=1}^T e^{-2C} \sum_{t=T/2}^T  \sum_{j=0}^{k_1-k - l} {t \choose j}{t \choose j+l}   \\
&\geq e^{-2C} \frac{T}{2}\sum_{j=0}^{k_1-k - l} {T/2 \choose j}{T/2 \choose j+l}  \\
&\geq C(k_1) T^{2k_1 - 2k -l +1}
\end{align}
and by a similar argument as before we get $B_{jk} = C(k_1)T^{2k_1-j-k +1}$. For brevity we use the same $C(k_1)$ to indicate different functions of $k_1$ as we are interested only in the growth with respect to $T$. To summarize
\begin{align}
B_{jk} &= C(k_1)T^{2k_1 - j - k +1} \label{jordan_value}
\end{align} 
whenever $T \geq 8d$. Recall Proposition~\ref{det_lb}, let the $M$ there be equal to $B$ then since 
\[
C_{ij} = C(k_1)\frac{B_{ij}}{\sqrt{B_{ii} B_{jj}}} = C(k_1)\frac{T^{2k_1 - j -k +1}}{\sqrt{T^{4k_1 - 2j - 2k + 2}}}
\]
it turns out that $C_{ij}$ is independent of $T$ and consequently $\lambda_{min}(C), \rho$ are independent of $T$ and depend only on $k_1$: the Jordan block size. Then $\prod_{j=1}^{k_1} B_{jj} \geq \text{det}(B) \geq \prod_{j=1}^{k_1} B_{jj} e^{-\frac{d\rho^2}{1 + \lambda_{\min}}} = C(k_1) \prod_{j=1}^{k_1} B_{jj}$. This means that $\text{det}(B) = C(k_1) \prod_{j=1}^{k_1} B_{jj}$ for some function $C(k_1)$ depending only on $k_1$. Further using the values for $B_{jj}$ we get
\begin{equation}
\label{det}
\text{det}(B) = C(k_1) \prod_{j=1}^{k_1} B_{jj} = \prod_{j=1}^{k_1} C(k_1) T^{2k_1 - 2l +1} = C(k_1) T^{k_1^2}
\end{equation}
Next we use Schur-Horn theorem, \textit{i.e.}, let $\sigma_i(B)$ be the ordered singular values of $B$ where $\sigma_i(B) \geq \sigma_{i+1}(B)$. Then $\sigma_i(B)$ majorizes the diagonal of $B$, \textit{i.e.}, for any $k \leq k_1$
\[
\sum_{i=1}^k \sigma_i(B) \geq \sum_{i=1}^{k} B_{ii}
\] 
Observe that $B_{ii} \leq B_{jj}$ when $i \leq j$. Then from Eq.~\eqref{jordan_value} it implies that
\begin{align*}
B_{k_1 k_1}=C_1(k_1)T &\geq \sigma_{k_1}(B) \\
\sum_{j=k_1-1}^{k_1} B_{jj} &= C_{2}(k_1)T^{3} + C_1(k_1)T \geq \sigma_{k_1 - 1}(A) + \sigma_{k_1}(A)
\end{align*}

Since $k_1 \geq 1$ it can be checked that for $T \geq T_1 =k_1\sqrt{\frac{C_1(k_1)}{C_2(k_1)}}$ we have $\sigma_{k_1-1}(A) \leq {(1+k_1^{-2})C_2(k_1)T^3} \leq {(1+k_1^{-1})C_2(k_1)T^3}$ as for every $T \geq T_1$ we have $C_2(k_1)T^3 \geq k_1^2C_1(k_1)T$. Again to upper bound $\sigma_{k_1-2}(A)$ we will use a similar argument
\begin{align*}
\sum_{j=k_1-2}^{k_1} B_{jj} &= C_3(k_1)T^{5} + C_2(k_1)T^{3} + C_1(k_1)T  \geq \sigma_{k_1-2}(A) +\sigma_{k_1-1}(A) + \sigma_{k_1}(A)
\end{align*}
and show that whenever 
\[
T \geq \max{\Big(T_1, k_1\sqrt{\frac{C_2(k_1)}{C_3(k_1)}}\Big)}
\]
we get $\sigma_{k_1-2}(A) \leq (1+k_1^{-2} + k_1^{-4}){C_3(k_1)T^5} \leq (1+k_1^{-1}){C_3(k_1)T^5}$ because $T \geq T_1$ ensures $C_2(k_1)T^3 \geq k_1^2C_1(k_1)T$ and $T \geq T_2 = k_1\sqrt{\frac{C_2(k_1)}{C_3(k_1)}}$ ensures $C_3(k_1)T^5 \geq k_1^2 C_2(k_1)T^3$. The $C_i(k_1)$ are not important, the goal is to show that for a sufficiently large $T$ we have an upper bound on each singular values (roughly) corresponding to the diagonal element. Similarly we can ensure for every $i$ we have $\sigma_i(A) \leq (1+k_1^{-1})C_{k_1 -i+1}(k_1)T^{2k_1 - 2i + 1}$, whenever 
\[
T > T_{i} = \max{\Big(T_{i-1}, k_1\sqrt{\frac{C_{i}(k_1)}{C_{i+1}(k_1)}}\Big)}
\]
Recall Eq.~\eqref{det} where $\text{det}(B) = C(k_1) T^{k_1^2}$. Assume that $\sigma_{k_1}(B) < \frac{C(k_1) T}{e \prod_{i=1}^d C_{i+1}(k_1)}$. Then whenever $T \geq \max{\Big(8d, \sup_{i}k_1\sqrt{\frac{C_{i}(k_1)}{C_{i+1}(k_1)}}\Big)}$
\begin{align*}
\text{det}(B) &= C(k_1) T^{k_1^2} \\
\prod_{i=1}^{k_1}\sigma_i &= C(k_1) T^{k_1^2} \\
\sigma_{k_1}(B)(1+k_1^{-1})^{k_1-1} T^{k_1^2-1}\prod_{i=2}^{k_1}C_{i+1}  &\geq C(k_1) T^{k_1^2} \\
\sigma_{k_1}(B) &\geq \frac{C_{k_1}T}{(1+k_1^{-1})^{k_1-1}\prod_{i=2}^{k_1}C_{i+1}} \\
&\geq \frac{C(k_1) T}{e \prod_{i=1}^{k_1} C_{i+1}(k_1)}
\end{align*}

which is a contradiction. This means that $\sigma_{k_i}(B) \geq \frac{C(k_1) T}{e \prod_{i=1}^{k_1} C_{i+1}(k_1)}$. This implies 
\[
\sigma_{\min}(\Gamma_T(A)) \geq 1 + \frac{\sigma_{\min}(P)^2}{\sigma_{\max}(P)^2} C(k_1)T
\]
for some function $C(k_1)$ that depends only on $k_1$.
\end{proof}	
It is possible that $\alpha(d)$ might be exponentially small in $d$, however for many cases such as orthogonal matrices or diagonal matrices $\alpha(A)=1$ [As shown in~\cite{simchowitz2018learning}]. We are not interested in finding the best bound $\alpha(d)$ rather show that the bound of Proposition~\ref{gramian_lb} exists and assume that such a bound is known. 

\begin{prop}
	\label{gramian_ratio}
Let $t_1/t_2 = \beta > 1$ and $A$ be a $d \times d$ matrix. Then 
\[
\lambda_1(\Gamma_{t_1}(A)\Gamma_{t_2}^{-1}(A)) \leq C(d, \beta)
\]
where $C(d, \beta)$ is a polynomial in $\beta$ of degree at most $d^2$ whenever $t_i \geq 8d$.
\end{prop}
\begin{proof}
	Since $\lambda_1(\Gamma_{t_1}(A)\Gamma_{t_2}^{-1}(A))  \geq 0$
	\begin{align*}
	\lambda_1(\Gamma_{t_1}(A)\Gamma_{t_2}^{-1}(A)) &\leq \text{tr}(\Gamma_{t_1}(A)\Gamma_{t_2}^{-1}(A)) \\
	&\leq  \text{tr}(\Gamma_{t_2}^{-1/2}(A)\Gamma_{t_1}(A)\Gamma_{t_2}^{-1/2}(A)) \\
	&\leq d \sigma_1(\Gamma_{t_2}^{-1/2}(A)\Gamma_{t_1}(A)\Gamma_{t_2}^{-1/2}(A)) \\
	&\leq d\sup_{||x|| \neq  0}\frac{x^{\prime} \Gamma_{t_1}(A) x}{x^{\prime}\Gamma_{t_2}(A) x}
	\end{align*}

Now 
\begin{align*}
\Gamma_{t_i}(A) &= P^{-1}\sum_{t=0}^{t_i} \Lambda^{t}PP^{\prime}(\Lambda^{t})^{*}P^{-1 \prime} \\
&\preceq  \sigma_{\max}(P)^2 P^{-1}\sum_{t=0}^{t_i} \Lambda^{t}(\Lambda^{t})^{*}P^{-1 \prime} \\
\Gamma_{t_i}(A) &\succeq  \sigma_{\min}(P)^2 P^{-1}\sum_{t=0}^{t_i} \Lambda^{t}(\Lambda^{t})^{*}P^{-1 \prime}
\end{align*}
Then this implies 
\[
\sup_{||x|| \neq  0}\frac{x^{\prime} \Gamma_{t_1}(A) x}{x^{\prime}\Gamma_{t_2}(A) x} \leq \frac{\sigma_{\max}(P)^2}{\sigma_{\min}(P)^2} \sup_{||x|| \neq  0}\frac{x^{\prime} \sum_{t=0}^{t_1} \Lambda^{t}(\Lambda^{t})^{*} x}{x^{\prime}\sum_{t=0}^{t_2} \Lambda^{t}(\Lambda^{t})^{*} x}
\]
Then from Lemma 12 in~\cite{abbasi2011improved} we get that
\[
\sup_{||x|| \neq  0}\frac{x^{\prime} \sum_{t=0}^{t_1} \Lambda^{t}(\Lambda^{t})^{*} x}{x^{\prime}\sum_{t=0}^{t_2} \Lambda^{t}(\Lambda^{t})^{*} x} \leq \frac{\text{det}(\sum_{t=0}^{t_1} \Lambda^{t}(\Lambda^{t})^{*})}{\text{det}(\sum_{t=0}^{t_2} \Lambda^{t}(\Lambda^{t})^{*})}
\]
Then 
\begin{align*}
\frac{\text{det}(\sum_{t=0}^{t_2} \Lambda^{t}(\Lambda^{t})^{*})}{\text{det}(\sum_{t=0}^{t_1} \Lambda^{t}(\Lambda^{t})^{*})} &\leq  \frac{\text{det}(\prod_{i=1}^l (\sum_{t=0}^{t_2} J_{k_i}(\lambda_i)^{t}(J_{k_i}(\lambda_i)^{t})^{*}))}{\text{det}(\prod_{i=1}^l(\sum_{t=0}^{t_1} J_{k_i}(\lambda_i)^{t}(J_{k_i}(\lambda_i)^{t})^{*}))}
\end{align*}
Here $l$ are the number of Jordan blocks of $A$. Then our assertion follows from Eq.~\eqref{det} which implies that the determinant of $\sum_{t=0}^{t_2} J_{k_i}(\lambda_i)^{t}(J_{k_i}(\lambda_i)^{t})^{*} $ is equal to the product of the diagonal elements (times a factor that depends only on Jordan block size), \textit{i.e.}, $C(k_i)t_2^{k_i^2}$. As a result the ratio is given by
\[
\frac{\text{det}(\prod_{i=1}^l (\sum_{t=0}^{t_2} J_{k_i}(\lambda_i)^{t}(J_{k_i}(\lambda_i)^{t})^{*}))}{\text{det}(\prod_{i=1}^l(\sum_{t=0}^{t_1} J_{k_i}(\lambda_i)^{t}(J_{k_i}(\lambda_i)^{t})^{*}))} = \prod_{i=1}^l \beta^{k_i^2}
\] 
whenever $t_2, t_1 \geq 8d$. Summarizing we get 
\[
\sup_{||x|| \neq  0}\frac{x^{\prime} \Gamma_{t_1}(A) x}{x^{\prime}\Gamma_{t_2}(A) x} \leq \frac{\sigma_{\max}(P)^2}{\sigma_{\min}(P)^2} \prod_{i=1}^l \beta^{k_i^2}
\]
\end{proof}

==> content/abstract.tex <==
%Machine Learning and Data Science (ML) is starting to take the place in industry that "Information Technology" had in the late 1990s: businesses of all sizes and in all sectors, are recognizing how necessary it has become to develop predictive capabilities for continued profitability of their core competencies. To be effective, ML algorithms rely on high-quality training data ? and not just any data, but data that is specific to the business problem that ML is applied to. Obtaining relevant training data can be very difficult for firms to do themselves, especially those early in their path towards incorporating ML into their operations. This problem is only further exacerbated, as businesses increasingly need to solve these prediction problems in real-time (e.g. a ride-share company setting prices, retailers/restaurants sending targeted coupons to clear inventory), which means that data gets ?stale? quickly. Therefore, it is imperative that there are real-time market structures for the buying and selling of training data for ML. Further it is insufficient to view ML performance metrics (e.g. RMSE) in isolation of real-world applications; for example, a $10\%$ increase in prediction accuracy means very different things for a hedge fund maximizing profits vs. a retailer decreasing inventory costs vs. a hospital trying to save lives. Hence the value of a dataset will necessarily have to consider more than simply the prediction accuracy it provides. Domain knowledge will be just as essential, if not more so, if we aim to view data as an asset and create a rigorous method to define its value. 

In this work, we aim to create a data marketplace; a robust matching mechanism to efficiently buy and sell data while optimizing social welfare and maximizing revenue. While the monetization of data and pre-trained models is an essential focus by many industries and vendors today, there does not exist a market mechanism that can price data and match buyers to vendors while still addressing the (computational and other) complexity associated with creating a market platform. The challenge in creating such a marketplace stems from the very nature of data as an asset: (i) it can be replicated at zero marginal cost; (ii) its value to a firm is inherently combinatorial (i.e. the value of a particular dataset depends on what other (potentially correlated) datasets are available); (iii) its value to a firm is dependent on which other firms get access to the same data; (iv) prediction tasks and the value of an increase in prediction accuracy vary widely between different firms, and so it is not obvious how to set prices for a collection of datasets with correlated signals; (v) finally, the authenticity and truthfulness of data is difficult to verify a priori without first applying it to a prediction task. Our proposed marketplace will take a holistic view of this problem and provide an algorithmic solution combining concepts from statistical machine learning, economics of data with respect to various application domains, algorithmic market design, and mathematical optimization under uncertainty. We will discuss some examples motivating this work. 





%We consider the task of interpolating and forecasting a time series in the presence of noise and missing data. 
%\iffalse % 
%Specifically, let 
%$f: \mathbb{Z} \to \mathbb{R}$ represent the latent discrete-time time series of interest. For each $t \in [0, T]$, with probability 
%$p \in (0, 1]$, we observe random variable $X(t)$ such that $\mathbb{E}[X(t)] = f(t)$, $X(t)$ are independent across
%$t$ and have uniformly bounded variance. The goal is to interpolate, i.e. estimate $f(t)$ for all $t \in [0, T]$ and forecast, i.e. estimate
%$f(T+1)$. 
%\fi
%As the main contribution of this work, we introduce an algorithm that transforms the observed time series into a 
%matrix, utilizes singular value thresholding to simultaneously recover missing values 
%and de-noise observed entries, and performs linear regression to make predictions. We argue that this method provides 
%meaningful imputation and forecasting for a large class of models: finite sum of harmonics (which approximate stationary
%processes), non-stationary sublinear trends, Linear Time-Invariant (LTI) systems, and their additive mixtures. In general, our algorithm recovers the hidden state of dynamics based on its noisy observations, like that of a Hidden Markov Model (HMM), provided the dynamics obey the above stated models. We demonstrate on synthetic and real-world datasets that our algorithm outperforms standard software packages not only in the presence of significantly missing data with high levels of noise, but also when the packages are given the underlying model while our algorithm remains 
%oblivious. This is in line with the finite sample analysis for these model classes.



==> content/bound_cross.tex <==
\subsection*{Bounding $C_T$}
In this section we will bound $C_T$ which includes the cross terms with noise and past state variables. We will show that with high probability this is only a small fraction of the total energy of the past terms. Specifically, recall
\begin{align*}
S_T &= \Gamma_T^{-1/2}\sum_{t=0}^{T-1} A x(t) x(t)^{'} A^{'} \Gamma_T^{-1/2} \\
C_T &= \sum_{t=0}^{T-1}\Gamma_T^{-1/2}Ax(t)\eta_{t+1}^{'}\Gamma_T^{-1/2}+ \Gamma_T^{-1/2}\eta_{t+1}x(t)^{'}A^{'}\Gamma_T^{-1/2}
\end{align*}
We want to show that $C_T + S_T \succeq (1 - \epsilon) S_T$. We will approach this by showing that $-\epsilon S_T \preceq C_T \preceq \epsilon S_T$. Formally, with high probability
\[
||S_T^{-1/2} C_T S_T^{-1/2}||_{\text{op}} < \epsilon
\]
Next, observe that $\hat{\eta}_t = \Gamma_T^{-1/2} \eta_t$, \textit{i.e.}, a transformed Gaussian vector with reduced variance. Before proving this we will need an essential result that is a variant (and stronger version) of Lemma 2 in~\cite{faradonbeh2017finite}. We defer the proof for later.
\begin{lem}
	\label{least_eigv}
	For a regular, explosive dynamical system, \textit{i.e.}, $\rho_{\min}(A) > 1$. If $T \geq C \log{\Big(\frac{-\log{\delta}}{\delta}\Big)}$ where $C$ is an absolute constant, then with probability at least $1-\delta$ it holds that,  
	\begin{align*}
	\rho_{\min}(\Gamma_T^{-1/2} Y_T \Gamma_T^{-1/2}) \geq \frac{c\phi(A)^2 \psi(A)^2\delta^2}{2}
	\end{align*}
\end{lem}
\begin{lem}
	\label{small_opnorm}
For any $v \in \Sc^{n}$ we have that 
\begin{align*}
\Pb(v^T S_T^{-1/2} C_T S_T^{-1/2} v )
\end{align*}
\end{lem}

==> content/conclusion.tex <==
%{\color{red} 
%Use Bose proposal for intro/conclusion. (1) Data needs to be valued. (2) Unique challenges - combinatorial, heterogeneous valuations, value changing in real-time. (3) Data Marketplace/Auction System is the way to go. \\
%
%Things left to do (In order of importance)
%\begin{enumerate}
%\item Bandits/Online Learning in a Metric Space
%	\begin{enumerate}
%		\item https://arxiv.org/pdf/0809.4882.pdf
%	\end{enumerate}
%\item Robustness to Replication of Data
%\item Multidimensional Myerson's Lemma 
%	\begin{enumerate}
%		\item http://www.sigecom.org/exchanges/volume_10/2/CAI.pdf
%	\end{enumerate} 
%\end{enumerate}
%}



==> content/document.tex <==
\section{Contributions}
\label{contribution}

==> content/dump_results.tex <==
\begin{lem}[Invertibility for Stable System]
	\label{stable_inversion}
	Define for any $0< \epsilon < 1/4$
	\begin{align*}
	T_1(\delta) &= \max{\Bigg\{768 \text{tr}(\Gamma_T-I)(2d \log{5} + \log{\frac{8}{\delta}}), \frac{16 (\gamma_T-1)^2 \text{tr}(\Gamma_T - I)}{c\text{tr}(\Gamma_{T/2}-I)^2} (\log{\frac{8}{\delta}} + 2d \log{5})\Bigg\}} \\
	T_2(\delta) &= 512\Big(\log{\dfrac{8}{\delta}} + d\log{5}\Big)\\
	T_3(\delta) &= \max{\{\frac{16 \beta_0 \gamma_0^2}{(1 -4 \epsilon)^2}, \frac{2 \text{tr}(\Gamma_T - I)}{\epsilon^2} \log{\frac{8d}{\delta}}  \}}
	\end{align*}
	For a stable $A$, and $T > \max\{T_1(\delta), T_2(\delta), T_3(\delta)\}$ we have probability at least $1 - \delta$,
	\[
	T P_1  \preceq Y_T \preceq T P_2
	\]
	where $P_1 = A P_1 A^{'} + \dfrac{7}{16}I, P_2 = A P_2 A^{'} + 2 I$.	
\end{lem}
\begin{proof}
	This result follows from a cute observation in~\cite{faradonbeh2017finite}. Observe that 
	\begin{align*}
	Y_T &=  x_0 x_0^{'} + A Y_T A^{'} + \\
	&+ \sum_{t=0}^{T-1}(A x_t\eta_{t+1}^{'} + \eta_{t+1}x_t^{'}A^{'}) + \sum_{t=1}^{T}\eta_t \eta_t^{'} \\
	&- Ax(T)x(T)^{'}A^{'}
	\end{align*}
	Define $\frac{1}{T} Y_T = \hat{Y}_T$. Then we can rewrite the preceding equation as 
	\begin{align}
	\hat{Y}_T &=  \frac{x_0 x_0^{'}}{T} + A \hat{Y}_T A^{'} + \nonumber\\
	&+ \sum_{t=0}^{T-1}\frac{(A x_t\eta_{t+1}^{'} + \eta_{t+1}x_t^{'}A^{'})}{T} + \sum_{t=1}^{T}\frac{\eta_t \eta_t^{'}}{T} \nonumber\\
	&- \frac{Ax(T)x(T)^{'}A^{'}}{T} \label{lyap_eq}
	\end{align}	
	
	
	From the preceding equality we will use the following lower and upper bounds respectively:
	\begin{equation}
	\label{lowerbnd_energy}
	\hat{Y}_T \succeq A \hat{Y}_{T-1} A^{\prime} + \sum_{t=0}^{T-1} \frac{Ax_t \eta_{t+1}^{\prime} + \eta_{t+1} x_t^{\prime} A^{\prime}}{T} + \sum_{t=1}^T \frac{\eta_t \eta_{t}^{\prime}}{T}
	\end{equation}
	%%%%%%%%%%%%%
	\begin{equation}
	\label{upperbnd_energy}
	\hat{Y}_T \preceq \frac{x_0 x_0^{\prime}}{T} + A \hat{Y}_T A^{\prime} + A\sum_{t=0}^{T-1} \frac{x_t \eta_{t+1}^{\prime} + \eta_{t+1} x_t^{\prime}}{T} A^{\prime} + \sum_{t=1}^T \frac{\eta_t \eta_{t}^{\prime}}{T}
	\end{equation}
	\subsection*{Bounding $\sum_{t=0}^{T-1}\frac{(A x_t\eta_{t+1}^{'} + \eta_{t+1}x_t^{'}A^{'})}{T}$}
	We want to show that the probability
	\[
	\Pb\Bigg(\bl \bl \sum_{t=0}^{T-1}\frac{(A x_t\eta_{t+1}^{'} + \eta_{t+1}x_t^{'}A^{'})}{T}\bl \bl \geq z \Bigg) 
	\]
	is small. To show this, observe
	\begin{align*}
	\Pb\Bigg(\bl \bl \sum_{t=0}^{T-1}\frac{(A x_t\eta_{t+1}^{'} + \eta_{t+1}x_t^{'}A^{'})}{T}\bl \bl \geq z \Bigg) &\leq \Pb\Bigg( \bl \bl \sum_{t=0}^{T-1}\frac{A x_t\eta_{t+1}^{'}}{T}\bl \bl \geq z/2\Bigg) \\
	&\leq 5^{2d} \Pb\Bigg(\bl \sum_{t=0}^{T-1}\frac{w^{\prime}A x_t\eta_{t+1}^{\prime} v}{T}\bl \geq z/8 \Bigg) \\
	&= 5^{2d} \Pb\Bigg(\bl\sum_{t=0}^{T-1}\frac{W_tZ_{t+1}}{T}\bl \geq z/8\Bigg)
	\end{align*}
	where $Z_t = \eta_{t}^{\prime} v, W_t = w^{\prime}A x_t$. Instead of $\Pb\Bigg(\bl\sum_{t=0}^{T-1}\frac{W_tZ_{t+1}}{T}\bl \geq z/8\Bigg)$, we analyze
	
	$$\Pb\Bigg(\bl\sum_{t=0}^{T-1}\frac{W_tZ_{t+1}}{T}\bl \geq z/8, \sum_{t=1}^T W_t^2 \leq \frac{3T}{2}\text{tr}(\Gamma_T)\Bigg)$$
	
	In Proposition~\ref{cumulative_energybnd} we substitute $\delta$ by $5^{-2d}\delta$ and for $T > \frac{16 (\gamma_T-1)^2 \text{tr}(\Gamma_T - I)}{c\text{tr}(\Gamma_{T/2}-I)^2}(\log{\frac{2}{\delta}} + 2d \log{5})$ we obtain 
	\begin{align*}
	\Pb\Bigg(\bl\sum_{t=0}^{T-1}\frac{W_tZ_{t+1}}{T}\bl \geq z/8, \sum_{t=1}^T W_t^2 \leq \frac{3T}{2}\text{tr}(\Gamma_T-1)\Bigg) + 5^{-2d}\delta &\geq \Pb\Bigg(\bl\sum_{t=0}^{T-1}\frac{W_tZ_{t+1}}{T}\bl \geq z/8\Bigg)
	\end{align*}
	Using Lemma~\ref{simchowitz_learning} we get 
	\begin{equation}
	\label{simchowitz_bnd}
	2 \exp{\Bigg(-\frac{Tz^2}{192 \text{tr}(\Gamma_T-I)}\Bigg)} +5^{-2d} \delta \geq \Pb\Bigg(\bl\sum_{t=0}^{T-1}\frac{W_tZ_{t+1}}{T}\bl \geq z/8\Bigg)
	\end{equation}
	
	
	Let 
	
	$$T_1(\delta) = \max{\Bigg\{768 \text{tr}(\Gamma_T-I)(2d \log{5} + \log{\frac{2}{\delta}}), \frac{16 (\gamma_T-1)^2 \text{tr}(\Gamma_T - I)}{c\text{tr}(\Gamma_{T/2}-I)^2} (\log{\frac{2}{\delta}} + 2d \log{5})\Bigg\}}$$
	
	then it easy to check that for $T > T_1(\delta)$ and $z=1/4$ in Eq.~\eqref{simchowitz_bnd}
	\[
	2 \exp{\Bigg(-\frac{T(1/4)^2}{192 \text{tr}(\Gamma_T-I)}\Bigg)} \leq 5^{-2d} \delta
	\]
	and we have 
	\begin{align*}
	\Pb\Bigg(\bl\sum_{t=0}^{T-1}\frac{W_tZ_{t+1}}{T}\bl \geq 1/32\Bigg) &\leq 5^{-2d} 2 \delta \\
	\Pb\Bigg(\bl \bl \sum_{t=0}^{T-1}\frac{(A x_t\eta_{t+1}^{'} + \eta_{t+1}x_t^{'}A^{'})}{T}\bl \bl \geq 1/4 \Bigg) &\leq 2 \delta
	\end{align*}
	
	For brevity, define $\Ec_1(\delta) = \Bigg\{T > T_1(\delta), \bl \bl \sum_{t=0}^{T-1}\frac{(A x_t\eta_{t+1}^{'} + \eta_{t+1}x_t^{'}A^{'})}{T}\bl \bl  \leq 1/4\Bigg\}$
	
	\subsection*{Bounding $\sum_{t=1}^T \frac{\eta_t \eta_t^{\prime}}{T}$}
	From Proposition~\ref{noise_energy_bnd} it follows that $\sum_{t=1}^T \frac{\eta_t \eta_t^{\prime}}{T}$ concentrates around $I$. We have, with probability at least $1 - \delta$, that 
	\begin{align*}
	||\dfrac{1}{T}\sum_{t=1}^T \eta_t \eta_t^{'} - I||  \leq \Bigg( \sqrt{\dfrac{32\Big(\log{\dfrac{2}{\delta}} + d\log{5})}{T}}\Bigg)
	\end{align*}
	Again we want $T$ large enough so that 
	\[
	\Bigg( \sqrt{\dfrac{32\Big(\log{\dfrac{2}{\delta}} + d\log{5})}{T}}\Bigg) \leq 1/4
	\]
	Then necessarily we have
	
	$$T \geq T_2(\delta) = 512\Big(\log{\dfrac{2}{\delta}} + d\log{5}\Big) $$ 
	
	For $T > T_2(\delta)$ we will have, with at least probability $1 - \delta$, that 
	\[
	\frac{3}{4} I \preceq \dfrac{1}{T}\sum_{t=1}^T \eta_t \eta_t^{'} \preceq \frac{5}{4}I
	\] 
	Define $\Ec_2(\delta) = \Bigg\{T \geq T_2(\delta),  \frac{3}{4} I \preceq \dfrac{1}{T}\sum_{t=1}^T \eta_t \eta_t^{'} \preceq \frac{5}{4}I\Bigg\}$
	
	\subsection*{Bounding $\frac{x(0) x(0)^{\prime}}{T} - \frac{Ax(T) x(T)^{\prime}A^{\prime}}{T}$}
	
	Since the initial condition is a constant, $\frac{x(0) x(0)^{\prime}}{T}$ decays linearly in $T$. From Assumption~\ref{bnd_init}, $\frac{||x(0) x(0)^{\prime}||}{T} \leq \frac{\gamma^2_0}{T}$. But for $\frac{Ax(T) x(T)^{\prime}A^{\prime}}{T}$ we use Proposition~\ref{stateOp_bnd}. From this we can conclude that 
	\begin{align}
	\Pb\Bigg(\frac{||Ax_T||_2}{\sqrt{T}} \geq \gamma + \frac{||A^{T+1}x_0||_2}{\sqrt{T}} \Bigg) &\leq 2d \exp\Big\{-\frac{T \gamma^2}{2 \text{tr}(\Gamma_T - I)}\Big\} \label{state_bnd}
	\end{align}
	
	Now, fix $0 < \epsilon < 1/4$. Then in Eq.~\eqref{state_bnd} we replace $\gamma = \frac{1}{4} - \frac{\beta_0 \gamma_0}{\sqrt{T}}$, and if $T > \frac{16 \beta_0 \gamma_0^2}{(1 -4 \epsilon)^2}$, we get 
	\begin{align}
	\Pb\Bigg(\frac{||Ax_T||_2}{\sqrt{T}} \geq 1/4 \Bigg) &\leq 2d \exp\Big\{-\frac{T\epsilon^2}{2 \text{tr}(\Gamma_T - I)}\Big\} \label{state_bnd2}
	\end{align}
	
	Define $T_3(\delta) = \max{\{\frac{16 \beta_0 \gamma_0^2}{(1 -4 \epsilon)^2}, \log{\frac{2d}{\delta}} \frac{2 \text{tr}(\Gamma_T - I)}{\epsilon^2}\}}$. Then, if $T > T_3(\delta)$, with probability at least $1 - \delta$ we have
	\[
	\frac{||Ax_T||_2}{\sqrt{T}} \leq 1/4
	\]
	
	Define $\Ec_3(\delta) = \Bigg\{T > T_3(\delta), \frac{||Ax_T||_2}{\sqrt{T}} \leq 1/4\Bigg\}$. 
	
	\subsection*{Event $\Ec_1(\delta) \cap \Ec_2(\delta) \cap \Ec_3(\delta)$}
	Since $\Pb(\Ec_1) \geq 1-2\delta, \Pb(\Ec_2) \geq 1-\delta, \Pb(\Ec_3) \geq 1-\delta$, we have $\Pb(\Ec_1(\delta) \cap \Ec_2(\delta) \cap \Ec_3(\delta)) \geq 1-4\delta$. 
	\vspace{3mm}
	Let $T_0 = \max\{T_1(\delta), T_2(\delta), T_3(\delta)\}$. Then for $T \geq T_0$ with probability at least $1 - 4 \delta$ we have 
	\begin{align*}
	\hat{Y}_T &=  \frac{x_0 x_0^{'}}{T} + A \hat{Y}_T A^{'}  \\
	&+ \sum_{t=0}^{T-1}\frac{(A x_t\eta_{t+1}^{'} + \eta_{t+1}x_t^{'}A^{'})}{T} + \sum_{t=1}^{T}\frac{\eta_t \eta_t^{'}}{T} \\
	&- \frac{Ax(T)x(T)^{'}A^{'}}{T} \\
	\hat{Y}_T &\succeq 0 + A \hat{Y}_T A^{'} \\
	&- \frac{1}{4}I + \frac{3}{4} I \\
	&- \frac{1}{16}I \\
	&= \frac{7}{16} I +  A \hat{Y}_T A^{'} 
	\end{align*}
	On the other hand, by a similar argument 
	\begin{align*}
	\hat{Y}_T &=  \frac{x_0 x_0^{'}}{T} + A \hat{Y}_T A^{'}  \\
	&+ \sum_{t=0}^{T-1}\frac{(A x_t\eta_{t+1}^{'} + \eta_{t+1}x_t^{'}A^{'})}{T} + \sum_{t=1}^{T}\frac{\eta_t \eta_t^{'}}{T} \\
	&- \frac{Ax(T)x(T)^{'}A^{'}}{T} \\
	\hat{Y}_T &\preceq 	 \frac{x_0 x_0^{'}}{T} + A \hat{Y}_T A^{'} \\
	&+\frac{1}{4}I + \frac{5}{4} I \\
	&\preceq 2I + A \hat{Y}_T A^{'}
	\end{align*}
	Define the following matrix solutions
	\begin{align*}
	P_1 &= A P_1 A^{'} + \dfrac{7}{16}I \\
	P_2 &= A P_2 A^{'} + 2I
	\end{align*}
	Then, for $T > T_0$, we have with probability at least $1- 4\delta$, $P_1 \preceq \bar{Y}_T \preceq P_2$.
	
	$$T P_1  \preceq Y_T \preceq T P_2$$
	
\end{proof}
Then, we have that

==> content/experiments.tex <==



==> content/explosive.tex <==
The concentration arguments used to show the convergence for stable systems does not work for unstable systems (contrary to what is suggested in~\cite{simchowitz2018learning}. The reason behind this is that the concentration results usually depend on the variance of $x_t$ which will scale as $\rho_{\max}^t$ and the such bounds become vacuous. On the other hand, based on anti--concentration results of martingales given in~\cite{}

It turns out that from a result of~\cite{nielsen2008singular} and later by~\cite{phillips2013inconsistent} that a notion of regularity is required for consistent estimation. For a linear system regularity implies that all eigenvalues of $A$ that have norm $ > 1$ should have geometric multiplicity of $1$. This leaves us to bound the square root of the inverse. 
Next, we use Lemma 2 in~\cite{faradonbeh2017finite} to show that $Y_{t}$ concentrates around $(A^t)(A^t)^{T}$ for large enough $t$. 
\begin{lem}
	\label{explosive}
Suppose that $\lambda_{\min}(A) > 1$; then there exists a constant $0 < \ell(A), \phi(A) < \infty$ such that
\[
\Pb(|\lambda_{\max}(A^{-n} Y_n (A^{T})^{-n})| > \ell(A) (-\log{\delta})) \leq \delta
\]
Further there is $c < \infty$ such that if $n \geq c \log{\big(- \log{\delta}/ \epsilon\big)}$, then with probability at least $1 - \delta$ it holds that 
\[
|\lambda_{\min}(A^{-n} Y_n (A^{T})^{-n})| > \phi(A) \delta^2 - \epsilon
\]
\end{lem}
From Lemma~\ref{explosive} we can conclude that $Y_t$ behaves as $A^t (A^T)^t$ with high probability. It is clear that $||(Y_T)^{-1/2}|| \leq C(A) |\lambda_{\min}|^{-T}/\delta$ which follows from~\cite{erxiong1994691}. We will use Lemma~\ref{explosive} to find a suitable $V$ matrix in Lemma~\ref{selfnorm_bnd}.
\begin{prop}
	\label{explosive_V}
	For any $T$ as in Lemma~\ref{explosive}, we have that with probability $1 - \delta/3$
	\begin{align*}
	(\phi(A)\delta^2/72)A^T (A^T)^{'} \preceq Y_T \preceq (-l(A)\log{\delta/6})( A^T (A^T)^{'} )
	\end{align*}
Define $\alpha(A, \delta) = (1 + 72/(\phi(A) \delta^2)), \beta(A, \delta) = (1 - \log{\delta/6})$. Then we have that with probability $1 - \delta$,
\[
||(\bar{Y}_{T})^{-1/2} \sum_{t=1}^T X_t \eta_t^T||^2_{\text{op}}\leq d\alpha(A, \delta)\log{\beta(A, \delta)} + \log{3/\delta}
\]
\end{prop}
\begin{proof}
	Pick $\epsilon = \phi(A)\delta^2/2$ in Lemma~\ref{explosive}. Then it can be checked that 
	\[
	A^{-n} Y_n (A^{-n})^{'} \succeq l(A)(- \log{\delta/6}) I 
	\]
	Using a similar argument for the lower bound we get our assertion. The proof of the rest follows by a similar argument as in Proposition~\ref{matrix_prop}.
\end{proof}	
\begin{cor}
	\label{convergence}
For a stable system, $\rho(A) \leq 1$, with probability $1 - \delta$ and for some absolute constant $C, C^{'}$
\[
T \geq C \log{3/\delta} + d \log{\Bigg(1 +  \dfrac{128\text{tr}(\Gamma_{\infty}(A))}{c^2 \sigma^2}\Bigg)}
\]
we have that 
\begin{align*}
||A - \hat{A}||_{\text{op}} &\leq (C^{'}/\sqrt{T})\sqrt{2(d\log{25 \gamma(A, \delta/3)}+ \log{3/\delta}) }
\end{align*}
where $\gamma(A, \delta/3) = \dfrac{\sigma^2 c^2/8 + \lambda_1(\Gamma_{\infty}(A), \delta/3)}{\sigma^2 c^2/8}$.

For an explosive system with probability $1 - \delta$, and for
\[
T \geq h(A) \log{1/\delta}
\]
where $h(A)$ is a system dependent constant, we have that 
\begin{align*}
||A - \hat{A}||_{\text{op}} &\leq \dfrac{(K |\lambda_{\min}(A)|^{-T})}{\delta}\sqrt{\alpha(A, \delta) d \log{\beta(A, \delta)} +  \log{1/\delta}}\\
&\leq (K^{'} \alpha^{'}(A)\dfrac{|\lambda_{\min}(A)|^{-T}}{\delta^2})\sqrt{ d \log{\beta(A, \delta)} +  \log{1/\delta}}
.\end{align*}
\end{cor}
We will now try to prove these results from first principle. We will focus on the set $\Wc = \{\sup_{1 \leq t \leq T} ||\eta_t||_{\infty} \leq \sqrt{2 \log{(Td/\delta)}}\}$. The reason is that we would like bound $x(t)$ at certain points to use familiar results of matrix martingales etc. Further, such a conditioning on subgaussian $\eta_t$ does not change independence and subgaussianity of $\eta_t$ under the new measure obtained by conditioning on $\Wc$. Our analysis will only deal with cases when $\rho(A) < 1$ and when the system is explosive, \textit{i.e.}, $|\lambda_{\text{min}}(A)| > 1$. 

\begin{align*}
V_T &= \sum_{t=0}^T\Gamma_{T}^{-1/2}  x(t)x(t)^{'}\Gamma_{T}^{-1/2} \\
&= \Gamma_T^{-1/2} x(0)x(0)^{'}\Gamma_{T}^{-1/2} + \sum_{t=0}^{T-1}\Gamma_{T}^{-1/2}  (Ax(t) + \eta_{t+1})(A x(t) + \eta_{t+1})^{'}\Gamma_{T}^{-1/2} \\
&= \Gamma_T^{-1/2} x(0)x(0)^{'}\Gamma_{T}^{-1/2} + \sum_{t=0}^{T-1}\Gamma_{T}^{-1/2} A x(t)x(t)^{'}A^{'}\Gamma_{T}^{-1/2} \\
&+ \Gamma_{T}^{-1/2}\sum_{t=0}^{T-1}(Ax(t)\eta_{t+1}^{'} + \eta_{t+1} x^{'}(t)A^{'})\Gamma_{T}^{-1/2} \\
&+ \Gamma_{T}^{-1/2} A (x(0)x(0)^{'} -  x(T)x(T)^{'})A^{'}\Gamma_{T}^{-1/2} \\
&+ \Gamma_T^{-1/2}\sum_{t=1}^{T} \eta_{t} \eta^{'}_{t} \Gamma_T^{-1/2}
\end{align*}
We will bound each of these terms step-by-step and attempt to show concentration. 
\begin{prop}
	\label{noise_var}
\[
\Pb(||(1/T)\sum_{t=1}^{T} \eta_{t} \eta^{'}_{t} - I||_{\text{op}} > t) \leq 2d\exp{-T t^2}
\]	
where each $\eta_t$ are random vectors with i.i.d. subgaussian entries.
\end{prop}	
Then it follows from Proposition~\ref{noise_var} that with probability $1 - 2d\exp{-T t^2}$
\[
T(1 - t) \Gamma^{-1}_T \preceq \Gamma_T^{-1/2}\sum_{t=1}^{T} \eta_{t} \eta^{'}_{t} \Gamma_T^{-1/2} \preceq T(1 + t) \Gamma^{-1}_T
\]

Defining 
\begin{align*}
\hat{A} &=\Gamma^{-1/2}_T A \Gamma^{1/2}_T \\
E_T &= \Gamma_T^{-1/2}\sum_{t=1}^{T} \eta_{t} \eta^{'}_{t} \Gamma_T^{-1/2} \\
D_T &= \Gamma_{T}^{-1/2} A (x(0)x(0)^{'} -  x(T)x(T)^{'})A^{'}\Gamma_{T}^{-1/2}\\
C_T &= \Gamma_{T}^{-1/2}\sum_{t=0}^{T-1}(Ax(t)\eta_{t+1}^{'} + \eta_{t+1} x^{'}(t)A^{'})\Gamma_{T}^{-1/2}\\
I_T &= \Gamma_T^{-1/2} x(0)x(0)^{'}\Gamma_{T}^{-1/2} \\
J_T &= \Gamma_{T}^{-1/2}\sum_{t=0}^{T-1}(Ax(t)\eta_{t+1}^{'} + \eta_{t+1} x^{'}(t)A^{'})\Gamma_{T}^{-1/2} + \sum_{t=0}^{T-1}\Gamma_{T}^{-1/2} A x(t)x(t)^{'}A^{'}\Gamma_{T}^{-1/2}
\end{align*}
The key step here is to show that $J_T$ remains positive semidefinite. It turns out that Lemma~\ref{explosive} is unavoidable, \textit{i.e.}, we need regularity of matrix $A$. The first point is that we will a modified noise term given by $\tilde{\eta}_t = \Gamma_T^{-1/2}\eta_t \sim \Nc(0, \Gamma_T^{-1})$. For any $u \in \Sc^{n-1}$, $\text{Variance}(\eta^T u) \leq ||\Gamma_T^{-1}||$. Next consider the following event where $Z_t = u^{'}Ax(t), \ell_t = u^{'} \eta_t$
\begin{align*}
\Sigma^s_T = \Bigg\{ \dfrac{\sum_{t=1}^T Z_t \ell_t}{\sqrt{\sum_{t=1}^T Z^2_t}} \geq \alpha, \sum_{t=1}^T Z^2_t \in [\beta_{-}, \beta_{+}]\Bigg\}
\end{align*}
Next consider the following event where $B_T = \sum_{t=1}^T \Gamma_T^{-1/2} A x(t) \tilde{\eta}^{'}_t +   \tilde{\eta}_t  x^{'}(t) A^{'} \Gamma_T^{-1/2}, F_T = \sum_{t=1}^T \Gamma_T^{-1/2} A x(t)x^{'}(t) A^{'} \Gamma_T^{-1/2} $
\begin{align*}
\Sigma^M_T = \Bigg\{ ||F_T^{-1/2} B_T F_T^{-1/2}||_{\text{op}} \geq \alpha^{'} \Bigg\}
\end{align*}
to note is that for any $u \in \Rb^n$
\[
|u^{'}\Gamma_{T}^{-1/2}\sum_{t=0}^{T-1}(Ax(t)\eta_{t+1}^{'} + \eta_{t+1} x^{'}(t)A^{'})\Gamma_{T}^{-1/2} u| \leq ||\Gamma_T^{-1/2}||_2 |u^{'}(\Gamma_{T}^{-1/2}\sum_{t=0}^{T-1}Ax(t)\eta_{t+1}^{'} + \eta_{t+1} x^{'}(t)A^{'}\Gamma_{T}^{-1/2})u|
\]

We already gave a concentration result for $E_T$. First we bound the quantity $\text{trace}(\Gamma_T^{-1/2} A x(t) x(t)^{'} A^{'} \Gamma_T^{-1/2})$. Let $\alpha_t = \Gamma_{T}^{-1/2} A x(t) x(t)^{'}A^{'} \Gamma_T^{-1/2}$
\subsection*{Bounding $\alpha_t$}
Here the hard step is to control the quantity
\[
\alpha_t =\Gamma_{T}^{-1/2} A x(t) x(t)^{'}A^{'} \Gamma_T^{-1/2}
\]
One way to deal with this is by observing that $x(t) = \sum_{s=0}^{t-1} A^{t-s} \eta_s$, then $\Gamma_{T}^{-1/2} A x(t) = \sum_{s=0}^t \Gamma_{T}^{-1/2} A^{t+1-s} \eta_s$. This can be written as 
\[
\Gamma_{T}^{-1/2} A x(t) = \sum_{j=1}^d \sum_{s=0}^t \Gamma_{T}^{-1/2} A^{t+1-s} e_j\eta_{sj}
\]
Now, we look at the Hermitian dilation of $\Gamma_{T}^{-1/2} A x(t)$ which is given by 
\[
\Hc(A x(t)) = \begin{bmatrix}
0 & \Gamma_{T}^{-1/2} A x(t) \\
x^{'}(t) A^{'} \Gamma_{T}^{-1/2} & 0 
\end{bmatrix}
\]
which can be written as 
\[
\Hc(A x(t)) = \sum_{j=1}^d \sum_{s=0}^{t} \eta_{sj}\begin{bmatrix}
0 & \Gamma_{T}^{-1/2} A^{t+1-s} e_j \\
e_j^{'} (A^{t+1-s})^{'} \Gamma_{T}^{-1/2} & 0 
\end{bmatrix}
\]
where $A_{sj} = \begin{bmatrix}
0 & \Gamma_{T}^{-1/2} A^{t+1-s} e_j \\
e_j^{'} (A^{t+1-s})^{'} \Gamma_{T}^{-1/2} & 0 
\end{bmatrix}$
Then it can be shown that 
$$
\sum_{s, j} A_{sj}^2 =  \begin{bmatrix}
\sum_{s=0}^{t} \Gamma_{T}^{-1/2} A^{t+1-s} (A^{t+1-s})^{'} \Gamma_{T}^{-1/2} & 0  \\
0  & \text{trace}(\sum_{s=0}^{t} \Gamma_{T}^{-1/2} A^{t+1-s} (A^{t+1-s})^{'} \Gamma_{T}^{-1/2})
\end{bmatrix}
$$
Here $\sigma_1(\sum_{s, j}A^2_{sj}) \leq \text{trace}(\Gamma_T^{-1/2} \Gamma_t \Gamma_T^{-1/2})$, then since we have $D_T$ in the form 
\[
D_t = \sum_{k} \gamma_k A_k
\]
where $A_k$ are fixed and $\gamma_k$ are i.i.d. subgaussian. We can bound the operator norm by results in~\cite{tropp2012user}, and this is of the form
\[
\Pb(||\alpha_t||_{\text{op}} > z) \leq 2d \exp{-\dfrac{z^2}{2 \text{trace}(\Gamma_T^{-1/2} \Gamma_t \Gamma_T^{-1/2})}}
\]
Observe the term $x_t = A^t x_0 + \sum_{\tau=1}^t A^{\tau-1} \eta_{\tau}$. One can alternately write this as
\begin{align*}
x_t &= \sum_{j=1}^d \sum_{s=0}^t  A^{t-s} e_j\eta_{sj} \\
x_t \eta_{t+1}^{'} &= \sum_{j=1}^d \sum_{s=0}^t  \eta_{sj} A^{t-s} e_j\eta_{t+1}^{'} \\
A x_t \eta_{t+1}^{'} &=  \sum_{j=1}^d\sum_{k=1}^d \sum_{s=0}^t  \eta_{sj}\eta_{t+1, k} A^{t+1-s} e_je_k^{'}
\end{align*}
The proof of our fact will hinge on bounding the operator norm of $Ax_t \eta_{t+1}^{'}$. Observe that $Ax_t \eta_{t+1}^{'}$ is a martingale difference sequence. Further, 


Now we give a concentration result for $C_T$.
\subsection*{Bounding $C_T$}
We work after conditioning under $\Wc$. Then let $Z_t = \Gamma_{T}^{-1/2}A x(t) \eta_{t+1}^{'} \Gamma_T^{-1/2}$, we have that almost surely
\[
C_T = \sum_{t=0}^{T-1} Z_t + Z_t^{'}
\]
$Z_t = uv^{'}$, then it is known that $uv^{'} + v u^{'} \succeq -uu^{'} - vv^{'}$ which follows from the fact that $(u+v)(u+v)^{'} \succeq 0$. Then $C_T \succeq \sum_{t=1}^T - Z_t Z_t^{'} - Z_t^{'} Z_t$. 
\begin{align*}
Z_t Z_t^{'} &= (\eta^{'}_{t+1}\Gamma_T^{-1} \eta_{t+1} )(\Gamma_{T}^{-1/2}A x(t) x^{'}(t) A^{'} \Gamma_{T}^{-1/2} )\\
Z_t^{'} Z_t &= (x(t)^{'}A^{'}\Gamma_T^{-1} A x(t))\Gamma_T^{-1/2} \eta_{t} \eta^{'}_{t} \Gamma_T^{-1/2}
\end{align*}
All noise terms are less that $\sqrt{2d \log{Td/\delta}}$ with probability at least $1 - \delta$.
\begin{lem}
	\label{noise_bnd}
	Under the event $\Wc$, we have that almost surely
	\[
		\eta_{t+1}^{'} \Gamma_T^{-1} \eta_{t+1} \leq 2d \log{(2Td/\delta)}\text{trace}(\Gamma_T^{-1})
	\]
\end{lem}
\begin{proof}
	This follows because we are working under the assumption that $||\eta_t||_{\infty} \leq \sqrt{\log{(2Td/\delta)}}$
\end{proof}	
\begin{lem}
	Under the event $\Wc$, we have that 
	\label{state_bnd}
	\[
	x(t)^{'}A^{'}\Gamma_T^{-1} A x(t) \leq \log{(2Td/\delta)}\text{trace}(\Gamma_T^{-1/2} \Gamma_t \Gamma_T^{-1/2})
	\]
\end{lem}
Lemma~\ref{noise_bnd},~\ref{state_bnd} suggest that whenever we have an explosive system. The term $Z_t Z_t^{'}$ is dominated by $\Gamma_T^{-1/2} Ax(t)x(t)^{'}A^{'}\Gamma_T^{-1/2}$. Further, $Z_t ^{'} Z_t$ then can be shown to concentrate around $\dfrac{2\log{Td}}{\delta^2}$, formally define $
N_T = \sqrt{2\log{Td}}/\delta \begin{bmatrix}
 \sqrt{\Gamma_T^{-1/2} \Gamma_1\Gamma_T^{-1/2}}\eta^{'}_1\\
 \vdots \\
 \sqrt{\Gamma_T^{-1/2} \Gamma_T\Gamma_T^{-1/2}}\eta^{'}_T
 \end{bmatrix}$

\begin{prop}
	\label{scale_noise}
Then $\Pb(||N_T||_{\text{op}} \geq \epsilon T) \leq 2d\exp{-\epsilon^2 T \delta / \log{T}}$
\end{prop}
The key conclusion here is that $C_T$ is dominated by the psd terms, \textit{i.e.}, $\sum_{t=1}^T \Gamma_T^{-1/2} \eta_t \eta_t^{'} + A x(t-1) x^{'}(t-1) A^{'} \Gamma_T^{-1/2} $. That is with high probability we can conclude that 
\[
V_T \succeq (1 - \epsilon) \sum_{t=1}^T \Gamma_T^{-1/2} \eta_t \eta_t^{'} + A x(t-1) x^{'}(t-1) A^{'} \Gamma_T^{-1/2} 
\]
As a result $s_{\min}(\sum_{t=0}^{T}x(t)x(t)^{'}) \geq \Omega(T)$. We have shown that the convergence for explosive systems is at least as fast as the stable system. A closer analysis would give us the exponential dependence, but this proof would not be very different from the analysis in Proposition 9~\cite{faradonbeh2017finite}. 
\begin{cor}
	\label{lower_bnd}
	There exists an absolute constant $C, C^{'}$ such that for $T  \geq (C/\delta)( \log{1/\delta} + d \log{d})$ we have that
	\[
	||A - \hat{A}||_{\text{op}} \leq (C^{'}/\sqrt{T})\sqrt{d \log{d /\delta}}
	\]
\end{cor}



==> content/general_bounds.tex <==
\section{General Bounds}
\label{gen_bounds}



==> content/market_construction.tex <==
% Explicit Construction 
We now explicitly construct instances of $\mathcal{AF}, \mathcal{PF}, \mathcal{PD}$ and $\mathcal{CF}$ and argue in Section \ref{sec:main_results} that the properties laid out in Section \ref{sec:marketplace_properties} hold for these particular constructions. \\

\textbf{Allocation Function.} Consider the following allocation function
\begin{align}\label{eq:alloc_function}
\mathcal{AF}^*(P_n, b_n) = \{m: m \in [M], \ b_n \ge P_n(m) \}
\end{align}
This particular $\mathcal{AF}$ allocates every feature, $m$, such that the marginal utility the buyer receives from an increase in prediction accuracy (i.e. $b_n$) is greater or equal to the marginal cost of feature, $P_n(m)$. To reduce notational overload, from here on out we overload $S_n = \mathcal{AF}(P_n, b_n)$ to refer both to the index of the features allocated (i.e. $S_n \subset [M]$) and the actual features themselves (i.e. $\bX_{S_n}$). \\

\textbf{Payment Function.} Consider the following payment function
\begin{align}\label{eq:payment_function}
\mathcal{PF}^*(P_n, b_n, Y_n)  = b_n \cdot \mathcal{G}(Y_n, \mathcal{M}(S_n)) - \int_{0}^{b_n} \mathcal{G}(Y_n, \mathcal{M}(\mathcal{AF}^*(z, P_n))) dz
\end{align}
This function is simply Myerson's payment rule constructed in \cite{Myerson_monotone_cost_rule}.  \\ 

\textbf{Payment-Division Function.} Let $\sigma_{S_n}$ refer to the set of all permutations over $S_n$ (the features allocated to buyer $n$). For any permutation $\sigma$ of $S_n$, let $[\sigma < m]$ refer to all the features in $S_n$ that came before $m$. We can now define our payment-divison function, $\mathcal{PD}$ explicitly in Algorithm \ref{alg-payment-division}. Note that $K \in \mathbb{N}$ is a hyperparameter that we provide guidance on how to pick in Section \ref{sec:main_results}. \\

\begin{algorithm}
\caption{- $\mathcal{PD}^*(S_n, Y_n, \mathcal{M}, \mathcal{G}, K, \mathcal{SM}, \lambda)$}\label{alg-payment-division}
\begin{algorithmic}[1]
\FORALL{$m \in S_n$}
	\FORALL{$k \in [K]$}
		\STATE $\sigma_k \sim \text{Unif}(\sigma_{S_n})$
		\STATE $G = \mathcal{G}(Y_n, \mathcal{M}(\bX_{[\sigma_k < m]})) $
		\STATE $G^+ = \mathcal{G}(Y_n, \mathcal{M}(\bX_{[\sigma_k < m \ \cup \ m]})) $
		\STATE $\hat{\psi}^k_n(m) = [G^+ - G]$
	\ENDFOR
	\STATE $\hat{\psi}_n(m) = \frac{1}{K} \sum^{K}_{k=1}\hat{\psi}^k_n(m)$
\ENDFOR
\STATE  $\psi_n(m) = \hat{\psi}_n(m)[(2+\epsilon) \sum^{S_n}_{m \neq j} S(X_m, X_j)]^{-1}$
\RETURN $\psi_n = [\psi_n(m) : m \in S_n]$
\end{algorithmic}
\end{algorithm} 

We now provide some intuition for this algorithm. The celebrated ``Shapley" value, $\psi_n$ (constructed in \cite{shapley_allocation}) is given by
\begin{equation}\label{eq:shapley_mechanism}
\psi_n(m) = \mathbb{E}_{\sigma \sim \text{Unif}(\sigma_{S_n})} [\mathcal{G}_n(Y_n, \mathcal{M}_n(\bX_{[\sigma < m \ \cup \ m]})) - \mathcal{G}_n(Y_n, \mathcal{M}_n(\bX_{[\sigma < m]})]
\end{equation}
It is well-known that the four conditions of Property \ref{prop:fair} are uniquely satisfied by the revenue division mechanism detailed in \eqref{eq:shapley_mechanism}. In words, \eqref{eq:shapley_mechanism} calculates the marginal contribution of feature $m$ to every subset of features, $S \in S_n  \setminus \{m\}$. Algorithm \ref{alg-payment-division} is a randomized analog of \eqref{eq:shapley_mechanism}, where instead of enumerating over all permutations in $\sigma_{S_n}$ (which has exponential complexity in $M$), we sample $\sigma_{k} \in \sigma_{S_n}$ uniformly at random with replacement, $K$ times. Finally, in order to enforce Condition 5 of Property \ref{prop:fair}, Algorithm \ref{alg-payment-division} does a post-processing (Step 10) which penalizes similar features (relative to the similarity metric, $\mathcal{SM}$). 
\\

\textbf{Price Update Algorithm.} The price update algorithm is essentially an online convex optimization, where the buyers (or nature) choose a convex cost function, \textit{i.e.}, negative of the payment function, at each time $n$. Algorithm~\ref{price-update-function} specifies the cost function $f_n(\cdot)$ at time $n$ as $-\mathcal{PF}(P_n, b_n, Y_n)$. We show in Lemma~\ref{lem:rev_convexity} that $f_n(\cdot)$ is convex in $P_n$.
\begin{algorithm}
	\caption{ - $ \mathcal{CF}(b_{n}, P_{n}, r_n, Y_n, n)$}\label{price-update-function}
	\begin{algorithmic}[1]
		\STATE $f_n(P_n) = -\mathcal{PF}(P_n, b_n, Y_n), g_n = \partial {f_n(P)}_{\{P=P_n\}}$ 
		\STATE $P^{'}_{n+1} = P_{n} - \eta_{n}g_{n}$ ($\eta_n$ is learning rate $\eta_{n-1} \geq \eta_{n} > 0$ )
		\STATE $P_{n+1} = \argmin_{P \in \mathcal{P}}||P - P^{'}_{n+1}||^2_2$
		\RETURN $P_{n+1}$
	\end{algorithmic}
\end{algorithm} 

Algorithm~\ref{price-update-function} is a version of OCO described in~\cite{zinkevich2003online} with subgradients. The projection step in Step 3 is to enforce that the price vectors come from a bounded step. The subgradients can be found by a simple polynomial time algorithm described in Proposition 7 of~\cite{hazan2012online}. 
\begin{equation}
\label{convex_price}
f_n(P_n) = \hat{f}_{\mathcal{G}}(P_n) + \infty \mathds{1}_{(P_n \not \in [0, b_n]^{M})}
\end{equation}

Since in Algorithm~\ref{price-update-function} we need to find the subgradients of a Lovasz extension

==> content/short_proof.tex <==
\section{Lower Bound for $Y_T$ when $A \in \Sc_0 \cup \Sc_1$}
\label{short_proof}
Here we will prove our results when $\rho(A) \leq 1+ C/T$. 
Define
\begin{align*}
P &= A Y_{T-1} A^{\prime} \\
Q &= \sum_{\tau=0}^{T-1}{Ax_t \eta_{t+1}^{\prime} }\\
V &= TI \\
T_{\eta} &= 512\Big(\log{\frac{2}{\delta}} + d \log{5}\Big) \\
\Ec_{1}(\delta) &= \Bigg\{||Q||^2_{(P+V)^{-1}} \leq 8 \log{\Bigg(\dfrac{5^d\text{det}(P+V)^{1/2} \text{det}(V)^{-1/2}}{\delta}\Bigg)}\Bigg\} \\
\Ec_{2}(\delta) &= \Bigg\{||\sum_{\tau=0}^{T-1} Ax_{\tau} x_{\tau}^{\prime}A^{\prime}|| \leq \frac{T \text{tr}(\Gamma_{T}(A) - I)}{\delta}\Bigg\}\\
\Ec_{\eta}(\delta) &= \{T > T_{\eta}(\delta), \frac{3}{4}I \preceq \dfrac{1}{T}\sum_{t=1}^T \eta_t \eta_t^{'} \preceq \frac{5}{4}I\} \\
\Ec(\delta) &= \Ec_{\eta}(\delta) \cap \Ec_{1}(\delta) \cap \Ec_{2}(\delta) \\
\end{align*}
Recall that
\begin{equation}
\label{lb_step1}
{Y}_T \succeq A {Y}_{T-1} A^{\prime} + \sum_{t=0}^{T-1} {Ax_t \eta_{t+1}^{\prime} + \eta_{t+1} x_t^{\prime}A^{\prime}} + \sum_{t=1}^T \eta_t \eta_t^{\prime}
\end{equation}

Our goal here will be to control
\begin{equation}
\label{cross_terms}
||Q||_2
\end{equation}
Following Proposition~\ref{selfnorm_bnd}, Proposition~\ref{energy_markov}, it is true that $\Pb(\Ec_{1}(\delta) \cap \Ec_{2}(\delta)) \geq 1-2\delta$. We will show that 
$$\Ec(\delta) = \Ec_{\eta}(\delta) \cap \Ec_{1}(\delta) \cap \Ec_{2}(\delta) \implies \sigma_{\min}(\hat{Y}_T) \geq 1/4$$
Under $\Ec_{\eta}(\delta)$, we get 
\begin{align}
{Y}_T &\succeq A {Y}_{T-1} A^{\prime} + \sum_{t=0}^{T-1} {Ax_t \eta_{t+1}^{\prime} + \eta_{t+1} x_t^{\prime}A^{\prime}} + \sum_{t=1}^T \eta_t \eta_t^{\prime} \nonumber \\
{Y}_T &\succeq A {Y}_{T-1} A^{\prime} + \sum_{t=0}^{T-1} {Ax_t \eta_{t+1}^{\prime} + \eta_{t+1} x_t^{\prime}A^{\prime}} + \frac{3}{4}TI  \nonumber \\
U^{\prime} {Y}_T U &\geq U^{\prime} A Y_{T-1} A^{\prime} U  + U^{\prime} \sum_{t=0}^{T-1} \Bigg({Ax_t \eta_{t+1}^{\prime} + \eta_{t+1} x_t^{\prime}A^{\prime}} \Bigg) U  + \frac{3}{4}T \hspace{3mm} \forall U\in \Sc^{d-1} \label{contra_eq}
\end{align} 
Intersecting Eq.~\eqref{contra_eq} with $\Ec_1(\delta) \cap \Ec_2(\delta)$, we find under $\Ec(\delta)$ 
\begin{align*}
&||Q||^2_{(P+V)^{-1}} \leq 8 \log{\Bigg(\dfrac{5^d\text{det}(P+V)^{1/2} \text{det}(V)^{-1/2}}{\delta}\Bigg)} \\
&\leq 8 \log{\Bigg(\dfrac{5^d \text{det}(\frac{T \text{tr}(\Gamma_{T}(A) - I)}{\delta} + TI)^{1/2}\text{det}(TI)^{-1/2}}{\delta}\Bigg)} \\
&\leq  8 \log{\Bigg(\dfrac{5^d \text{det}({ \text{tr}(\Gamma_{T}(A) - I)} + I)^{1/2}}{\delta^d}\Bigg)} 
\end{align*}
Using Proposition~\ref{psd_result_2} and letting $\kappa^2 = U^{\prime} P U$ then 
\begin{align*}
&||QU||_2 \\
&\leq \sqrt{\kappa^2 + T}\sqrt{8 \log{\Bigg(\dfrac{5^d \text{det}({ \text{tr}(\Gamma_{T}(A) - I)} + I)^{1/2}}{\delta^d}\Bigg)}}
\end{align*}
So Eq.~\eqref{contra_eq} implies 
\begin{align}
U^{\prime} {Y}_T U &\geq \kappa^2 \nonumber - \sqrt{(\kappa^2 + T)}{ \sqrt{ 16d \log{( \text{tr}(\Gamma_T - I)+1)} + 32d \log{\frac{5}{\delta}}}} + \frac{3}{4}T 
\end{align}
which gives us
\begin{align}
U^{\prime} \frac{{Y}_T}{T} U &\geq \frac{\kappa^2}{T} - \sqrt{(\frac{\kappa^2}{T} + 1)}\underbrace{ \sqrt{ \frac{16d}{T} \log{( \text{tr}(\Gamma_T - I)+1)} + \frac{32d}{T}\log{\frac{5}{\delta}}}}_{=\beta} + \frac{3}{4} \label{contra_eq2}
\end{align}
If we can ensure
\begin{equation}
\label{t_req}
\frac{T}{128} \geq  { \frac{d}{2} \log{( \text{tr}(\Gamma_T - I)+1)} + d \log{\frac{5}{\delta}} }
\end{equation}
then $\beta \leq 1/2$, \textit{i.e.}, 
\[
 \sqrt{ \frac{16d}{T} \log{( \text{tr}(\Gamma_T - I)+1)} + \frac{32d}{T}\log{\frac{5}{\delta}}} \leq \frac{1}{2}
\]
Let $T$ be large enough that Eq.~\eqref{t_req} is satisfied then Eq.~\eqref{contra_eq2} implies
\begin{equation}
\label{final_eq}
U^{\prime} \frac{{Y}_T}{T} U \geq \frac{\kappa^2}{T} - \frac{\sqrt{(\frac{\kappa^2}{T}  + 1)}}{2} + \frac{3}{4} \geq \frac{1}{4} + \frac{\kappa^2}{2T}
\end{equation}

Since $U$ is arbitrarily chosen Eq.~\eqref{final_eq} implies
\begin{align}
Y_T \succeq \frac{T}{4}I \label{lower_bnd}
\end{align}
with probability at least $1 - 3\delta$ whenever
\begin{align}
\rho_i(A) &\leq 1 + \frac{c}{T} \nonumber\\
T &\geq \max{\Big(512\Big(\log{\frac{2}{\delta}} + d \log{5}\Big), 128\Big({ \frac{d}{2} \log{( \text{tr}(\Gamma_T - I)+1)} + d \log{\frac{5}{\delta}} }\Big)\Big)} \label{t_req_comb}
\end{align}
%%%%%%%
\begin{remark}
Eq.~\eqref{t_req} is satisfied whenever $\text{tr}(\Gamma_T - I)$ grows at most polynomially in $T$. This is true whenever $\rho(A) \leq 1 +\frac{c}{T}$. 
\end{remark}


==> content/subsidiary_results.tex <==
Observe that $x_t = \sum_{s=1}^{t} A^{t-s} \eta_s + A^t x_0$ where $x_0$ is the initial condition. We can express this as 
\[
x_t = \sum_{j=1}^d \sum_{s=1}^{t} A^{t-s} e_j \eta_{sj}  + A^{t} x_0
\]
where $\{e_j\}$ is the canonical basis. 
\begin{prop}
	\label{stateOp_bnd}
	For a matrix $A$, we have 
		\[
		\Pb(||x_t - A^{t}x_0||_2 \geq z) \leq 2 d \exp{-\dfrac{z^2}{2\text{trace}(\Gamma_{t-1})}}
		\]
	Then with probability at least $1 - \delta/K$ we have 
	$$||x_t - A^t x_0||_2 \leq \sqrt{2 \text{trace}(\Gamma_{t-1}) \log{\dfrac{2Kd}{\delta}}}$$ 
	
	Further, with probability at least $1 - \delta$ we have
	$$\sup_{t \leq T} ||x_t - A^t x_0||_2 \leq \sqrt{2 \text{trace}(\Gamma_{T-1}) \log{\dfrac{2Td}{\delta}}}$$

\end{prop}
\begin{proof}
	From Theorem 4.1 in~\cite{tropp2012user}, we know that for self--adjoint $B_k$
	\[
	\Pb(||\sum_{k} \gamma_k B_k|| \geq \alpha) \leq 2d \exp{-\alpha^2/2\sigma^2}
	\]
	where $\gamma_k$ are i.i.d Gaussian, $\sigma^2 = ||\sum_k B_k^2||$. Recall that 
	\[
	\beta_t = x_t - A^{t} x_0= \sum_{j=1}^d \sum_{s=1}^{t} A^{t-s} e_j \eta_{sj}  
	\]
	We will instead find the operator norm of $\Hc(\beta_t)$ where 
		\[
		\Hc(\beta_t) = \sum_{j=1}^d \sum_{s=1}^{t} \eta_{sj} \begin{bmatrix}
		0 & A^{t-s} e_j \\
		e_j^{'}(A^{t-s})^{'} & 0 
		 \end{bmatrix}    
		\]
		Then $$\sigma^2 = ||\sum_{j=1}^d \sum_{s=1}^{t} \begin{bmatrix}
		0 & A^{t-s} e_j \\
		e_j^{'}(A^{t-s})^{'} & 0 
		\end{bmatrix}^2|| =  ||\sum_{s=1}^{t} \sum_{j=1}^d \begin{bmatrix}
		 A^{t-s} e_j e_j^{'} A^{t-s} & 0\\
		0& \text{trace}(A^{t-s} e_j e_j^{'} A^{t-s}) 
		\end{bmatrix}||  $$
	Now, 
	\begin{align*}
	||\sum_{s=1}^{t} \sum_{j=1}^d \begin{bmatrix}
	A^{t-s} e_j e_j^{'} A^{t-s} & 0\\
	0& \text{trace}(A^{t-s} e_j e_j^{'} A^{t-s}) 
	\end{bmatrix}|| &= ||\sum_{s=1}^{t}  \begin{bmatrix}
	A^{t-s} \sum_{j=1}^d e_j e_j^{'} A^{t-s} & 0\\
	0& \text{trace}(A^{t-s}  \sum_{j=1}^d e_j e_j^{'} A^{t-s}) 
	\end{bmatrix}|| \\
	&= ||  \begin{bmatrix}
\sum_{s=1}^{t}	A^{t-s}  A^{t-s} & 0\\
	0& \text{trace}(\sum_{s=1}^{t} A^{t-s}  A^{t-s}) 
	\end{bmatrix}||
	\end{align*}
	This gives $\sigma^2 = \text{trace}(\Gamma_{t-1})$. We have shown that $||\beta_t||_2$ is a subgaussian random variable.
	
	The last assertion will follow from the fact that we are finding the maxima of $T$ subgaussian random variables.
\end{proof}	
\begin{prop}
	\label{noise_energy_bnd}
	Let $\eta_t$ be i.i.d Gaussian vectors. Then for every $z \in (0, 1)$
	\begin{align*}
	\Pb(||\dfrac{1}{T}\sum_{t=1}^T \eta_t \eta_t^{'} - I|| \geq z) \leq 2 \cdot 5^d \exp{-T\frac{z^2}{32} }
	\end{align*}
	Then with probability at least $1 - \delta$,
	\[
	||\dfrac{1}{T}\sum_{t=1}^T \eta_t \eta_t^{'} - I||  \leq  \sqrt{\dfrac{32\Big(\log{\dfrac{2}{\delta}} + d\log{5})}{T}} 
	\]
\end{prop}
\begin{assumption}
	\label{noise}
We will assume that all probabilities in this section are conditioned on the event $\Wc$, where 
\[
\Wc = \Bigg\{\sup_{t}||\eta_t||_{\infty} \leq \sqrt{2 \log{\dfrac{Td}{\delta}}}\Bigg\}
\]
\end{assumption}
\begin{prop}
	\label{subg_bnd}
	Under the event $\Wc$, $||\eta_t||_2 \leq \sqrt{2d \log{\dfrac{Td}{\delta}}}$ almost surely. Further, $\eta_t$ are i.i.d subgaussian random vectors under the event $\Wc$, \textit{i.e.},
	\[
	\Pb(\eta_1 \in A_1, \ldots, \eta_t \in A_T | \Wc) = \prod_{s=1}^t \Pb(\eta_s \in A_s| \Wc) 
	\]
\end{prop}
Proposition~\ref{subg_bnd} is a useful tool that allows us to bound the state variables and use existing matrix concentration results. 
\begin{prop}
	\label{stateGamma_bnd}
Let $x_t$ be the state vector at time $t$ generated by a LTI system with state transition matrix $A$. Then
\[
\Pb\Bigg(||x_t||_2 \leq  \gamma_t  \sqrt{2d \log{\dfrac{Td}{\delta}}} | \Wc\Bigg) = 1
\]
\end{prop}
We want to bound the quantity 
\[
||(\Xb^T \Xb)^{+} \Xb^T E||_2
\]
We provide a simplified analysis of this case here
\begin{align*}
||(\Xb^T \Xb)^{+} \Xb^T E||_2 &\leq ||((\Xb^T \Xb)^{+})^{1/2}||_2||((\Xb^T \Xb)^{+})^{1/2} \Xb^T E||_2 \\
&= ||(Y_T^{+})^{1/2}||_2 ||(Y_T^{+})^{1/2} \sum_{t=1}^T X_t \eta_t^T||_2
\end{align*}
Recall that $Y_T$ is the cumulative state energy at time $T$. 
%Define $\tilde{S}_T = \sum_{t=1}^T X_t \eta_t^T$ then it turns out that $(Y_T^{+})^{1/2}\tilde{S}_T$ is self--normalized. 
%%%%%
\begin{remark}
	We will attempt to show invertibility of $\Xb^{T}\Xb$ without a small ball argument. The case for explosive systems will require a nuanced argument as the control required for a small ball type argument is not possible.
\end{remark}
%%%%%%
\begin{prop}[\cite{vershynin2010introduction}]
	\label{eps_net}
We have for any $\epsilon < 1$ and any $w \in \Sc^{d-1}$ that 
\[
\Pb(||(Y_T^{+})^{1/2} \sum_{t=1}^T X_t \eta_t^T|| > z) \leq (1 + 2/\epsilon)^d \Pb(||(Y_T^{+})^{1/2} \sum_{t=1}^T X_t \eta_t^Tw|| > \frac{z}{2})
\]
\end{prop}
Proposition~\ref{eps_net} helps us in using the tools developed in de la Pena et. al. and~\cite{abbasi2011improved} for self--normalized martingales. We will define $S_t = \sum_{\tau=1}^t X_{\tau} \tilde{\eta}_{\tau}$ where $\tilde{\eta}_t=w^T \eta_t$ is standard normal. Specifically, we use Lemma 9 of~\cite{abbasi2011improved} which we state here for convenience
\begin{thm}[Theorem 3~\cite{abbasi2011improved}]
	\label{selfnorm_main}
Let $\{\tilde{\eta}_t, S_t, \bcF_t \}_{t=1}^{T}$ be defined as before. Let $\tau$ be a stopping time w.r.t $\{\bcF_t\}$. Then for any $0 < \delta < 1$  with probability $1 - \delta$ we have 

\[
||S_{\tau}||^2_{\bar{Y}^{-1}_{\tau}} \leq 2 \log{\Bigg(\dfrac{\text{det}(\bar{Y}_{\tau})^{1/2} \text{det}(V)^{-1/2}}{\delta}\Bigg)}
\]
where $\bar{Y}^{-1}_{\tau} = (Y_{\tau} + V)^{-1}$ and $V$ is deterministic with $V \succ 0$.
\end{thm}
\begin{cor}
	\label{selfnorm_bnd}
	For any $0 < \delta < 1$ and $\{\eta_t, S_t, \bcF_t \}_{t=1}^{T}$ defined as before, we have with probability $1 - \delta$
	\[
	||(\bar{Y}_{T})^{-1/2} \sum_{t=1}^T X_t \eta_t^T||_2 \leq \sqrt{8d \log {\Bigg(\dfrac{5 \text{det}(\bar{Y}_{T})^{1/2d} \text{det}(V)^{-1/2d}}{\delta^{1/d}}\Bigg)}}
	\]
where $\bar{Y}^{-1}_{\tau} = (Y_{\tau} + V)^{-1}$ and any deterministic $V$ with $V \succ 0$.
\end{cor}

Lemma~\ref{selfnorm_bnd} gives us a way to control the norm of $S_T$. Unfortunately we do not know for what $V$ get the best bound. A key observation is the following:
\begin{prop}
	\label{matrix_prop}
Given $V = \lambda I \succ 0$ and a vector $S$ which lies in the subspace spanned by the rows of positive semi--definite matrix $Y$, we have
\[
||S||_{(V +Y)^{-1}} \geq  \inf_{1 \leq i \leq d, \sigma^{Y}_i > 0}\dfrac{\sigma^{Y}_i}{\lambda + \sigma^{Y}_i} ||S||_{Y^{+}}
\]
Here $\sigma_i^Y$ is the $i^{th}$ singular value of $Y$ and $\sigma_i^Y \geq \sigma_{i+1}^Y$.
\end{prop}
\begin{proof}
	The proof follows by simple linear algebra. Let $Y = U \Sigma^Y U^T$ where $\sigma_i^Y$ is the $i^{th}$ singular value of $Y$. For a vector $S = \sum_{i=1}^d \lambda_i u_i$,  where $u_i$ are the eigenvectors of $Y$. Note that $\lambda_i = 0$ if the eigenvalue corresponding to $u_i$ is $0$. 
	\[
	S^T (V + Y)^{-1} S = \sum_{i=1}^d \lambda_i^2 (\sigma_i + \lambda)^{-1}
	\]
	Similarly, if $\sigma_K$ is the least eigenvalue that is greater than $0$ we have
		\[
		S^T Y^{+} S = \sum_{i=1}^K \lambda_i^2 \sigma_i^{-1}
		\]
	and the claim follows in a straightforward way.
\end{proof}	
